Best-Buddies Tracking

Best-Buddies Tracking (BBT) applies the Best-Buddies Similarity measure (BBS) to the problem of model-free online tracking. BBS was introduced as a similarity measure between two point sets and was shown to be very effective for template matching. Originally, BBS was designed to work with point sets of equal size, and we propose a modification that lets it handle point sets of different size. The modified BBS is better suited to handle scale changes in the template size, as well as support a variable number of template images. We embed the modified BBS in a particle filter framework and obtain good results on a number of standard benchmarks.

==> introduction.tex <==
\section{Introduction}
Online tracking plays an important role in many computer vision applications such as autonomous driving, surveillance systems and human-computer-interface, to name a few. Tracking is a challenging task because of changes in view-point, illumination and non rigid deformations of the object to be tracked. A tracker must strike a delicate balance between adapting to legitimate changes in the appearance of an object and adapting to background clutter thus causing drift.

These sources of variability require a representation that is invariant to them or the development of similarity measures that can handle them. In its most basic form, online tracking boils down to template matching, where the goal is to find a given template in the current image. This requires the definition of a similarity measure, such as minimizing the intensity difference between the template and the target. To complicate things, it is common to represent the position of an object with a bounding box. The bounding box often include some background pixels and this can hurt the matching function and cause drift.

We address these problems by using a new (dis)similarity measure called the Best-Buddies Similarity or BBS \cite{DekelEtAl15}. BBS is used within a standard particle filter algorithm, and the resulting tracker is termed the Best-Buddies Tracker or BBT.

The template and candidate image regions are mapped to two point sets in some high dimensional space where BBS takes place. The mapping simply involves breaking the image region into small patches and creating vectors (i.e., high dimensional points) consisting of their pixel value and relative $xy$ position. BBS counts the number of Best-Buddies Pairs (BBPs) - pairs of points in source and target sets, where each point is the nearest neighbor of the other. This simple measure is quite robust to geometric deformations and considerable amount of outliers, making it an ideal candidate for tracking. 

BBS, as formulated in \cite{DekelEtAl15}, applies to point sets of arbitrary size. In general one would expect BBS to be invariant to set size. This is a desired property in the context of visual tracking where point sets may have different size due to scale changes or use of multiple templates for example. Unfortunately, we find BBS not to be invariant to set size. Specifically, our analysis shows that BBS score increases if one set is increased in size while the other is kept fixed. We analyze this phenomenon both theoretically and empirically, and suggest several ways to address the problem. 

Key to our solutions is the understanding that in order for BBS to be consistent the size of both sets must be equal. We therefore propose both a clustering and a random sampling scheme as pre-processing stages before the BBS computation and show that both solve the problem.    

In the original work BBS was used for template matching and was evaluated exhaustively using a sliding window approach. In BBT we propose incorporating BBS into a particle filtering framework removing the need to perform an exhaustive search and allowing us to account for scale changes as well.

A single template is not enough to capture the variability in the appearance of an object over time and modern trackers often use multiple templates. We extend BBS to deal with temporally varying data, by augmenting data from points taken from multiple templates and also address the question of why using this ``bag-of-points'' representation makes sense.

In the spirit of best buddies pairs approach we assess the confidence of the tracker by a forward-backward consistency check. This information is mainly used for template update purposes. Inspired by Kalal et al. \cite{Kalal2010}, our  forward-backward consistency check verifies that tracking from the current frame backward will arrive at the position of the object in some previous reference frame.

In order to make the tracker more robust to scale changes we use an ensemble of several independent BBT trackers, with different scale parameters. The results from these trackers is then fused using a recently published fusion technique.  

We perform extensive tests evaluating the performance of BBT using three common benchmarks. Performance is compared with other recently published methods and demonstrates good initial performance. A closer look at the performance envelope reveals that better performance can potentially be achieved by better tracker fusion.
 
To summarize, the contribution of our work is two fold: (i) We address the problem of computing BBS with unbalanced point sets. We analyze the problem both theoretically and empirically, and propose two effective solutions to the problem. (ii) We propose a novel tracking framework termed BBT that uses BBS as a similarity measure. We perform extensive experiments evaluating its performance and comparing them to other recently published methods showing promising initial results. 
